Common Representation of Information Flows for Dynamic Coalitions

We propose a formal foundation for reasoning about access control policies within a Dynamic Coalition, defining an abstraction over existing access control models and providing mechanisms for translation of those models into information-flow domain. The abstracted information-flow domain model, called a Common Representation, can then be used for defining a way to control the evolution of Dynamic Coalitions with respect to information flow.

==> eptcsdata.tex <==
\providecommand{\event}{Jeremy W. Bryans and John S. Fitzgerald (Eds.): \\
Formal Aspects of Virtual Organisations 2009 (FAVO2009)}
\providecommand{\volume}{16}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{15}
\providecommand{\eid}{2}
\pdfoutput=1

